Enhancing JEPAs with Spatial Conditioning: Robust and Efficient Representation Learning

Image-based Joint-Embedding Predictive Architecture (IJEPA) offers an attractive alternative to Masked Autoencoder (MAE) for representation learning using the Masked Image Modeling framework. IJEPA drives representations to capture useful semantic information by predicting in latent rather than input space. However, IJEPA relies on carefully designed context and target windows to avoid representational collapse. The encoder modules in IJEPA cannot adaptively modulate the type of predicted and/or target features based on the feasibility of the masked prediction task as they are not given sufficient information of both context and targets. Based on the intuition that in natural images, information has a strong spatial bias with spatially local regions being highly predictive of one another compared to distant ones. We condition the target encoder and context encoder modules in IJEPA with positions of context and target windows respectively. Our "conditional" encoders show performance gains on several image classification benchmark datasets, improved robustness to context window size and sample-efficiency during pretraining.

==> sections/deprecated/todos.tex <==
\section{To Dos}
\etai{should we use the timm or reference based model family? both?} \newline
\anand{My opinion would be to stick to reference based model family as it makes comparisons a lot easier to judge based on the controls $\rightarrow$ only difference between models would be the conditioning aspect. It's more beneficial to show that the conditional encoders continue to show gains at scale (model capacity: ViT-B/L/H and pre-training compute: 300 v/s 600 epochs) than have many model versions.} \newline
\vimal{if we can get results for all models we care about in timm family then we can consider this model as an option. The numbers we are able to obtain for ViT-L is higher and almost a match with the numbers published in I-JEPA. See third bullet point in StoP repo~\footnote{https://github.com/amirbar/StoP?tab=readme-ov-file\#differences-compared-to-the-official-i-jepa-implementation} for potential differences between what is included in public repo and implementation used in I-JEPA publication.}
\begin{enumerate}
    \item get numbers for imagenet on VIT-B/L (maybe H?) \etai{some tasks are running for VIT-L. next week once we have more gpus we'll run everything}
    \item get numbers for imagenet on ViT-B/L for the robustness to context window
    \item get numbers for clever (\anand{im on this})
    \item numbers for OOD sets (\anand{im on this})
    \item robustness experiments (context size mainly)
    \item Understand if its worth it to include numbers for the robotics benchmarks
    \item motivational experiments - game environment (\etai{im on this})
    \item a theoretical motivation (\etai{im on this})
\end{enumerate}

==> sections/related-work.tex <==
\section{Related Work}

